Standardized Non-Intrusive Reduced Order Modeling Using Different Regression Models With Application to Complex Flow Problems

In recent years, numerical methods in industrial applications have evolved from a pure predictive tool towards a means for optimization and control. Since standard numerical analysis methods have become prohibitively costly in such multi-query settings, a variety of reduced order modeling (ROM) approaches have been advanced towards complex applications. In this context, the driving application for this work is twin-screw extruders (TSEs): manufacturing devices with an important economic role in plastics processing. Modeling the flow through a TSE requires non-linear material models and coupling with the heat equation alongside intricate mesh deformations, which is a comparatively complex scenario. We investigate how a non-intrusive, data-driven ROM can be constructed for this application. We focus on the well-established proper orthogonal decomposition (POD) with regression albeit we introduce two adaptations: standardizing both the data and the error measures as well as -- inspired by our space-time simulations -- treating time as a discrete coordinate rather than a continuous parameter. We show that these steps make the POD-regression framework more interpretable, computationally efficient, and problem-independent. We proceed to compare the performance of three different regression models: Radial basis function (RBF) regression, Gaussian process regression (GPR), and artificial neural networks (ANNs). We find that GPR offers several advantages over an ANN, constituting a viable and computationally inexpensive non-intrusive ROM. Additionally, the framework is open-sourced to serve as a starting point for other practitioners and facilitate the use of ROM in general engineering workflows.

==> Highlights.tex <==
% From https://www.elsevier.com/authors/journal-authors/highlights :
"Highlights are three to five (three to four for Cell Press articles) bullet points that help increase the discoverability of your article via search engines. These bullet points should capture the novel results of your research as well as new methods that were used during the study (if any). [..] Please include terms that you know your readers will be looking for online. Don't try to capture all ideas, concepts or conclusions as highlights are meant to be short: 85 characters or fewer, including spaces. [..] No jargon, acronyms, or abbreviations: aim for a general audience and use keywords. [..] Consider the reader - Highlights are the first thing they'll see. "

%% I think the highlights should aim to explain some keywords in the title and direct interest towards the abstract. Probably ok to be slightly provocative and not simply 'reformulate' the title too much.
% Should mention POD, ANN, GPR, RBF, 'explain' standardization and complex flow problems

% each highlight must be under 85 characters including whitespaces which is this much
0000000000000000000000000000000000000000000000000000000000000000000000000000000000000

% this would be one idea:
Proper orthogonal decomposition with three different regression models is used
Neural networks, Gaussian process- and radial basis function regression are compared
Standardization steps aid interpretability and reusability of the method
Time is treated discretely similar to space for computational efficiency
Time- and temperature-dependent, (non-)Newtonian flow is studied

Proper orthogonal decomposition with three different regression models is used
Standardization steps aid interpretability and reusability of the method
Time is treated discretely similar to space for computational efficiency
Time- and temperature-dependent, (non-)Newtonian flow is studied
Gaussian process regression offers several advantages over artificial neural networks

% Here are some alternatives
Non-intrusive reduced basis method is applied to three different flow problems
Gaussian process regression offers several advantages over artificial neural networks
Time is treated discretely similar to space for computational efficiency
Problems are parametrized in domain geometry and material properties
Steady, unsteady, simple and generalized Newtonian fluid flow problems are considered
Time- and temperature-dependent flow of a generalized Newtonian fluid is also studied

% each highlight must be under 85 characters including whitespaces which is this much
0000000000000000000000000000000000000000000000000000000000000000000000000000000000000
